Towards Bug-Free Distributed Go Programs

Programmers of distributed systems need to reason about concurrency to avoid races. However, reasoning about concurrency is difficult, and unexpected races show up as bugs. Data race detection in shared memory systems is well-studied (dynamic data race detection [13], behavioral types [15], dynamic race detection [31]). Similar to how a data race consists of reads and writes not related by happens-before at a shared memory location, a communication race consists of receives and sends not related by happens-before on a shared channel. Communication races are problematic: a receiver expects a specific message from a specific sender, but with a communication race, the receiver can receive a message meant for another receiver, or not receive anything at all. In this work, we describe a verification framework that can prove the absence of communication races for distributed programs that use a subset of the Go programming language, where synchronization is mainly achieved via message passing. We statically reason about how a distributed program executes, using a happens-before order, extended to buffered and unbuffered channels.

==> figures/projection_functions_figure.tex <==
\begin{figure}
  {\centering
    \only<+>{ \begin{subfigure}[t]{\textwidth}
      \begin{subequations}
        \begin{align}
          &\projectOntoP{\transmit{\Party'}{\channel{c'}{\anything}}{i}{\Party''}}{\Party} &&= \begin{cases}
            \Ep{\Party'}{i} \CB{\channel{c'}{\anything}} &\text{if $\Party = \Party'$} \\
            \CB{\channel{c'}{\anything}} \Ep{\Party''}{i} &\text{if $\Party = \Party''$} \\
            \emp &\text{otherwise} \\
          \end{cases} \tag{Transmission} \\
          &\text{For some fixed $\channel{d}{0}$,} \notag \\
          &\projectOntoP{\guardP{\Ep{\Party'}{i} \HB{} \Ep{\Party''}{j}}}{\Party} &&= \begin{cases}
            \guardP{\channel{d}{0}, \Ep{\Party'}{i}} \ssep \Ep{\Party'}{k} \CB{\channel{d}{0}} &\text{if $\Party = \Party'$, for some $k > i$} \\
              \CB{\channel{d}{0}} \Ep{\Party''}{h} \ssep \guardP{\channel{d}{0}, \Ep{\Party''}{j}} &\text{if $\Party = \Party''$, for some $h < j$} \\
                \emp &\text{otherwise} \\
              \end{cases} \tag{Guard} \\
          &\projectOntoP{\emp}{\Party} &&= \emp \tag{Inaction} \\
          &\projectOntoP{\GlobalProtocol_1 \ssep \GlobalProtocol_2}{\Party} &&= \projectOntoP{\GlobalProtocol_1}{\Party} \ssep \projectOntoP{\GlobalProtocol_2}{\Party} \tag{Sequence} \\
          &\projectOntoP{\GlobalProtocol_1 \asep \GlobalProtocol_2}{\Party} &&= \projectOntoP{\GlobalProtocol_1}{\Party} \asep \projectOntoP{\GlobalProtocol_2}{\Party} \tag{Concurrency}
        \end{align}
      \end{subequations}
      \caption{The projection function that projects global protocols onto party $\Party$ to obtain per-party protocols.}
      \label{fig:global to per-party projection}
    \end{subfigure} }

    \only<+>{ \begin{subfigure}[t]{\textwidth}
      \begin{subequations}
        \begin{align}
          \projectOntoP{\Ep{\Party'}{i} \CB{\channel{c'}{\anything}}}{\Channel} &= \begin{cases}
            \Ep{\Party'}{i} \CB{} &\text{if $\Channel = \channel{c'}{\anything}$} \\
            \emp &\text{otherwise} \\
          \end{cases} \tag{Send} \\
          \projectOntoP{\CB{\channel{c'}{\anything}} \Ep{\Party'}{i}}{\Channel} &= \begin{cases}
            \CB{} \Ep{\Party'}{i} &\text{if $\Channel = \channel{c'}{\anything}$} \\
            \emp &\text{otherwise} \\
          \end{cases} \tag{Receive} \\
          \projectOntoP{\guardP{\channel{d}{\anything}, \Ep{\Party'}{i}}}{\Channel} &= \begin{cases}
            \guardP{\Ep{\Party'}{i}} &\text{if $\Channel = \channel{d}{\anything}$} \\
            \emp &\text{otherwise} \\
          \end{cases} \tag{Guard} \\
          \projectOntoP{\emp}{\Channel} &= \emp \tag{Inaction} \\
          \projectOntoP{\GlobalProtocol_1 \ssep \GlobalProtocol_2}{\Channel} &= \projectOntoP{\GlobalProtocol_1}{\Channel} \ssep \projectOntoP{\GlobalProtocol_2}{\Channel} \tag{Sequence} \\
          \projectOntoP{\GlobalProtocol_1 \asep \GlobalProtocol_2}{\Channel} &= \projectOntoP{\GlobalProtocol_1}{\Channel} \asep \projectOntoP{\GlobalProtocol_2}{\Channel} \tag{Concurrency}
        \end{align}
      \end{subequations}
      \caption{The projection function that projects per-party protocols onto endpoint $\Channel$ to obtain per-endpoint protocols.}
      \label{fig:per-party to per-endpoint projection}
    \end{subfigure} }
    \caption{The projection functions.}
    \label{fig:projection functions}
  }
\end{figure}


==> figures/satisfaction_with_and_without_races_figure.tex <==
\begin{figure}
  {\centering
    \begin{tikzpicture}[scale=0.55,every node/.style={transform shape}]]
      \draw (0,0) node[draw,circle,minimum size=3cm,label=above:programs with races] (ImplsWithRaces) {};
      \draw (0,-7) node[draw,circle,minimum size=3cm,label=below:race-free programs] (ImplsRaceFree) {};
      \draw (7,0) node[draw,circle,minimum size=3cm,label=above:protocols with races] (ProtsWithRaces) {};
      \draw (7,-7) node[draw,circle,minimum size=3cm,label=below:race-free protocols] (ProtsRaceFree) {};

      % satisfaction
      \draw [-Implies,double distance=5pt] (ImplsWithRaces) -- (ProtsWithRaces) node [above,near start,fill=white,inner sep=1pt] {satisfies};
      \draw [-Implies,double distance=5pt] (ImplsRaceFree) -- (ProtsRaceFree) node [above,near start,fill=white,inner sep=1pt] {satisfies};
      \draw [-Implies,double distance=5pt] (ImplsRaceFree) -- (ProtsWithRaces) node [above,near start,fill=white,inner sep=1pt] {satisfies};

      % transformation
      \draw [-triangle 90] (ProtsWithRaces) -- (ProtsRaceFree) node [text width=3cm,right,near start,fill=white,inner sep=1pt] {transformation described in section \ref{sec:Transforming Global Protocols with Races into Race-free Global Protocols}};

      % elements
      \draw (0,0) node[draw,circle,inner sep=1mm,fill=black,label=above:Program \ref{lst:simple global protocol implementation}] (ImplsWithRacesElem) {};
      \draw (0,-7) node[draw,circle,inner sep=1mm,fill=black,label=above:Program \ref{lst:simple global protocol guarded implementation}] (ImplsRaceFreeElem) {};
      \draw (7,0) node[draw,circle,inner sep=1mm,fill=black,label=above:Protocol \eqref{eq:global protocol with races}] (ProtsWithRacesElem) {};
      \draw (7,-7) node[draw,circle,inner sep=1mm,fill=black,label=above:Protocol \eqref{eq:global protocol race-free}] (ProtsRaceFreeElem) {};
    \end{tikzpicture}
    \caption{\label{fig:satisfaction with and without races}
      This figure shows two sets of programs, and two sets of protocols.
      Examples of protocol conformance and protocol transformation are concretely shown for one element of each set.
      Although our verification framework can verify protocol conformance (where protocol conformance is shown by a double arrow labelled ``satisfies'' from some set of programs to some set of protocols, and an example of conformance is that the program \ref{lst:simple global protocol implementation} in this figure satisfies the protocol with races \eqref{eq:global protocol with races} in this figure), users of our framework may want to verify that their Go program has more interesting properties than just protocol conformance.
      To this end, users should provide a richer specification which captures more interesting properties, such as race-freedom.
      Users can apply the transformation described in section \ref{sec:Transforming Global Protocols with Races into Race-free Global Protocols} to any protocol with races (e.g. \eqref{eq:global protocol with races}), to automatically obtain a new race-free protocol (e.g. \eqref{eq:global protocol race-free}) that communicates similarly to the old protocol with races.
      This transformation is shown by a single arrow from the set of protocols with races to the set of race-free protocols.
      Users can then make corrections to their original Go program, so that the program is race-free (e.g. \ref{lst:simple global protocol implementation} is corrected to \ref{lst:simple global protocol guarded implementation})
      Users can then use our verification framework to verify that the corrected race-free program (e.g. \ref{lst:simple global protocol guarded implementation}) satisfies a race-free protocol (e.g. \eqref{eq:global protocol race-free}).
      Furthermore, our verification framework can also verify that the corrected race-free program (e.g. \ref{lst:simple global protocol guarded implementation}) also satisfies the old protocols with races (e.g. \eqref{eq:global protocol with races}).
    }
  }
\end{figure}


==> figures/verification_rules_and_lemmas_figure.tex <==
\begin{figure}
  \only<+>{ \begin{subfigure}[t]{\textwidth}
    {\centering
      \begin{subequations}
        \begin{align}
          \GlobalProtocol &\implies \PartyProtocolPredicate{\Party}{\projectOntoP{\GlobalProtocol}{\Party}} \asep \PartyProtocolPredicate{\Party'}{\projectOntoP{\GlobalProtocol}{\Party'}} \asep \ldots &&\text{for some parties $\Party, \Party', \ldots$} \label{eq:Global to Per-party} \tag{Global to Per-party} \\
          \PerPartyProtocol &\implies \EndpointProtocolPredicate{\Channel}{\projectOntoP{\PerPartyProtocol}{\Channel'}} \asep \EndpointProtocolPredicate{\Channel}{\projectOntoP{\PerPartyProtocol}{\Channel'}} \asep \ldots &&\text{for some endpoints $\Channel, \Channel', \ldots$} \label{eq:Per-party to Per-endpoint} \tag{Per-party to Per-endpoint}
        \end{align}
      \end{subequations}
      \caption{Projection lemmas.}
      \label{fig:projection lemmas}
    }
  \end{subfigure} }

  \only<+>{ \begin{subfigure}[t]{\textwidth}
    {\centering
      \begin{subequations}
        \begin{align}
          \Rule
          {}
          {\triple
          {\EndpointProtocolPredicate{\Channel}{\ChannelSend{\Ep{\Party}{i}} \cdot \EndpointProtocolPredicate{\channel{c'}{\anything}}{\PerEndpointProtocol'} \ssep \PerEndpointProtocol} \asep \EndpointProtocolPredicate{\channel{c'}{\anything}}{\PerEndpointProtocol'}}
          {c <- c'}
          {\EndpointProtocolPredicate{\Channel}{\PerEndpointProtocol} \land \Ep{\Party}{i}}
          }&
             \label{eq:Endpoint Send} \tag{Endpoint Send} \\
          \Rule
          {}
          {\triple
          {\EndpointProtocolPredicate{\Channel}{\ChannelReceive{\Ep{\Party}{i}} \cdot \EndpointProtocolPredicate{\channel{c'}{\anything}}{\PerEndpointProtocol'} \ssep \PerEndpointProtocol}}
          {c' := <-c}
          {\EndpointProtocolPredicate{\Channel}{\PerEndpointProtocol} \asep \EndpointProtocolPredicate{\channel{c'}{\anything}}{\PerEndpointProtocol'} \land \Ep{\Party}{i}}
          }&
             \label{eq:Endpoint Receive} \tag{Endpoint Receive} \\
          \Rule
          {}
          {\triple
          {\EndpointProtocolPredicate{\Channel}{\ChannelSend{\Ep{\Party}{i}} \ssep \PerEndpointProtocol}}
          {c <- *}
          {\EndpointProtocolPredicate{\Channel}{\PerEndpointProtocol} \land \Ep{\Party}{i}}
          }&
             \label{eq:Data Send} \tag{Data Send} \\
          \Rule
          {}
          {\triple
          {\EndpointProtocolPredicate{\Channel}{\ChannelReceive{\Ep{\Party}{i}} \ssep \PerEndpointProtocol}}
          {<-c}
          {\EndpointProtocolPredicate{\Channel}{\PerEndpointProtocol} \land \Ep{\Party}{i}}
          }&
             \label{eq:Data Receive} \tag{Data Receive}
        \end{align}
      \end{subequations}
      \caption{Hoare triple rules.}
      \label{fig:Hoare triple rules}
    }
  \end{subfigure} }

  \only<+>{ \begin{subfigure}[t]{\textwidth}
    {\centering
      \begin{subequations}
        \begin{align}
          (\guardP{\Psi} \ssep \text{Protocol}) \land \Psi &\implies \text{Protocol} \land \Psi \label{eq:Prove Guard} \tag{Prove Guard}
        \end{align}
      \end{subequations}
      \caption{A lemma that proves a guard, where Protocol is either $\GlobalProtocol$, $\PerPartyProtocol$, or $\PerEndpointProtocol$.}
      \label{fig:prove guard lemma}
    }
  \end{subfigure} }

  \only<+>{ \begin{subfigure}[t]{\textwidth}
    {\centering
      \begin{subequations}
        \begin{align}
          \EndpointProtocolPredicate{\Channel}{\PerEndpointProtocol} \asep \EndpointProtocolPredicate{\Channel'}{\PerEndpointProtocol'} \asep \ldots &\implies \PartyProtocolPredicate{\Party}{\PerEndpointProtocol \asep \PerEndpointProtocol' \asep \ldots} \notag \\
          \text{for some endpoints $\Channel, \Channel', \ldots$ of some party $\Party$} \label{eq:Per-endpoint to Per-party} \tag{Per-endpoint to Per-party}
        \end{align}
      \end{subequations}
      \caption{Unprojection lemma, where residues of each endpoint are joined together.}
      \label{fig:unprojection lemma}
    }
  \end{subfigure} }
  \caption{Verification rules and lemmas.}
  \label{fig:verification rules and lemmas}
\end{figure}


==> header.tex <==
\newcommand{\emp}{\texttt{emp}}
\newcommand{\HB}[1]{\prec_{HB}^{#1}}
\newcommand{\CB}[1]{\prec_{CB}^{#1}}
\newcommand{\E}[1]{E^{#1}}
\newcommand{\Party}{P}
\newcommand{\GlobalProtocol}{G}
\newcommand{\PerPartyProtocol}{\Pi}
\newcommand{\PerEndpointProtocol}{\zeta}
\newcommand{\Ep}[2]{{#1}^{#2}} % event belonging to a party
\newcommand{\channel}[2]{
  % identifier, capacity
  {{#1}^{#2}}
}

\newcommand{\triple}[3]{\{#1\}\ \texttt{#2}\ \{#3\}}
\newcommand{\hoareAssert}[1]{\{#1\}}

%\makeatletter
%
%\newcommand*\IsExactlyOneToken[1]{%
%  TT\fi
%  \ifx\@empty#1\@empty
%    \expandafter\@EmptyCase
%  \else
%    \expandafter\@IsOnlyOneToken
%  \fi
%  #1\@@@
%}
%\@ifdefinable\@IsOnlyOneToken{\def\@IsOnlyOneToken#1#2\@@@{%
%  \ifx\@empty#2\@empty
%}}
%\@ifdefinable\@EmptyCase{\def\@EmptyCase#1\@@@{% #1 for robustness
%  \iffalse % since 0 != 1
%}}
%
%\makeatother
%
%\newcommand{\EndpointProtocolPredicate}[2]{
%  % channel, protocol
%  \mathcal{C}(#1,
%  \if\IsExactlyOneToken{#1}
%    #2
%  \else
%    (#2)
%  \fi
%  )
%}

\newcommand{\EndpointProtocolPredicate}[2]{
  % channel, protocol
  \mathcal{C}(#1, (#2))
}
\newcommand{\ChannelSend}[1]{
  % event
  #1 \CB{}
}
\newcommand{\ChannelReceive}[1]{
  % event
  \CB{} #1
}
\newcommand{\PartyProtocolPredicate}[2]{
  % party, protocol
  \mathcal{P}(#1, (#2))
}
\newcommand{\PartySend}[2]{
  % channel, event
  #2 \CB{#1}
}
\newcommand{\PartyReceive}[2]{
  % channel, event
  \CB{#1} #2
}

\newcommand{\Rule}[2]{\genfrac{}{}{0.7pt}{}{{\setlength{\fboxrule}{0pt}\fbox{$#1$}}}{{\setlength{\fboxrule}{0pt}\setlength{\fboxsep}{3mm}\fbox{$#2$}}}}

\newcommand{\anything}{\ast}
\newcommand{\party}[1]{#1}
\newcommand{\transmit}[4]{{#1} \xrightarrow[#2]{#3} {#4}}

\newcommand{\Channel}{\channel{c}{\anything}}

\usepackage{xifthen}
\newcommand{\kw}[1]                              {\mathrel{\mathtt{#1}}}
\newcommand{\sds}                               {\kw{sd}}
\newcommand{\rvs}                               {\kw{rv}}
% dop for option with duration
\newcommand\dop[6][]{
  % ?, name, label, pos-x, pos-y, label-pos
  \draw [fill] (#4+0.05,#5) arc (0:180:0.05) -- cycle;
  \draw [fill] (#4-0.05,#5-0.3) arc (180:360:0.05) -- cycle;
  \draw [fill] (#4-0.05,#5) rectangle node (#2s) {} ++(0.1, 0.001);
  \draw [fill] (#4-0.05,#5-0.3) rectangle node (#2e) {} ++(0.1, 0.001);
  \draw [] (#2s.center) -- (#2e.center)
  node [#6=2mm, midway] (1) {#3};
}
% dop for option with duration
\newcommand\doplength[7][]{
  % ?, name, label, pos-x, pos-y, label-pos, length
  \draw [fill] (#4+0.05,#5+#7) arc (0:180:0.05) -- cycle;
  \draw [fill] (#4-0.05,#5-0.3) arc (180:360:0.05) -- cycle;
  \draw [fill] (#4-0.05,#5+#7) rectangle node (#2s) {} ++(0.1, 0.001);
  \draw [fill] (#4-0.05,#5-0.3) rectangle node (#2e) {} ++(0.1, 0.001);
  \draw [] (#2s.center) -- (#2e.center)
  node [#6=2mm, midway] (1) {#3};
}
% pop for point operation
\newcommand\pop[6][]{
  % ?, name, label, pos-x, pos-y, label-pos
  \draw [fill] (#4,#5) circle [radius=0.05] node (#2) {}
  node [#6=2.5mm] (1) {#3};
}
\newcommand{\sdop}[3]{%
  \ifthenelse{\isempty{#3}}%
    {\sds^{#1}\ {#2}}%
    {\sds^{#1}\ {#2}\ {#3}}%
}
\newcommand{\rvop}[3]{%
  \ifthenelse{\isempty{#3}}%
    {\rvs^{#1}\ {#2}}%
    {\rvs^{#1}\ {#2}\ {#3}}%
}
\newcommand{\wrop}[2]                           {{#1}!{#2}}
\newcommand{\rdop}[2]                           {{#1}?{#2}}

\usepackage[utf8]{inputenc}
\usepackage{amsmath,amssymb,amsfonts,amsthm,textcomp}
\usepackage[font=footnotesize]{caption}
\usepackage{setspace}
\usepackage{hyperref}
\usepackage{fancyref}
\usepackage{makecell,adjustbox,tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usepackage{indentfirst}

\usepackage[numbers]{natbib}
\let\parencite\citep
\let\parencites\citep
\let\textcite\citet

\usepackage{xcolor}
\definecolor{greencyan}{rgb}{0.5, 1.0, 0.83}
\definecolor{marine}{rgb}{0.0, 0.5, 1.0}
\definecolor{firebrick}{rgb}{0.7, 0.13, 0.13}

\usepackage{listings,lstautogobble,multicol}

\lstset{
  autogobble=true,
  mathescape=true,
  escapechar=\%,
  language=Go,
  basicstyle=\ttfamily\footnotesize,
  commentstyle=\color{gray}\textit,
  escapebegin=\color{gray}, % Assume escaped LaTeX is always in comment
  keywordstyle=\color{firebrick},
  numberstyle=\color{marine},
  stringstyle=\color{greencyan},
  captionpos=b,
  numbers=left,
}

\lstnewenvironment{code}[1][]%
{\singlespacing
  \noindent\minipage{\linewidth}
  \lstset{
    #1 % pass newenvironment options to lstlisting
  }
}
{\onehalfspacing
  \endminipage}

\usepackage{thmtools}
\newtheorem{conj}{Conjecture}
\newtheorem{req}{Requirement}
\newtheorem*{weak}{Weak Ordering}

\usepackage{caption}
\usepackage{subcaption}
\usepackage{newfloat}
\newcounter{enumcnt}
\DeclareFloatingEnvironment[name={List}]{enumcnt}

\usepackage{mathtools}
\DeclarePairedDelimiter\parens{\lparen}{\rparen}
\DeclareMathOperator{\receiveOfSend}{\CB{\Channel}}
\DeclareMathOperator{\projectOnto}{\downharpoonright}
\DeclareMathOperator{\guard}{\ominus}
\DeclareMathOperator{\ssep}{;}
\DeclareMathOperator{\asep}{\ast}
\newcommand{\receiveOfSendP}[1]{\receiveOfSend\parens*{#1}}
\newcommand{\projectOntoP}[2]{\parens*{#1}\projectOnto_{#2}}
\newcommand{\guardP}[1]{\guard\parens*{#1}}

\usepackage{enumitem}
\setlist[description]{font=\boldmath\bfseries,leftmargin=!,labelwidth=\widthof{\boldmath\bfseries \text{$\guardP{\Ep{\Party}{i} \HB{} \Ep{\Party'}{i}}$}}} % TODO hardcoded labelwidth

\tolerance=1
\emergencystretch=\maxdimen
\hyphenpenalty=10000
\hbadness=10000

\setlength\parskip{1em plus 0.1em minus 0.2em}
\setlength\parindent{0pt}

\newcommand{\mytextsim}{\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$} \,}

\title{
  Towards Bug-Free Distributed Go Programs
}
\author{Koo Zhengqun}
\date{April 23, 2021}

% \numberwithin{table}{section}


==> lstlistings/simple_global_protocol_guarded_implementation_lstlisting_overlay1.tex <==
\begin{lstlisting}[label={lst:simple global protocol guarded implementation},multicols=2]
package main

var c = make(chan int, 2)
var d = make(chan int, 0)
var e = make(chan int, 0)

func main() {
        go A()
        go B()
        go C()
}

func A() {
        c <- 1
        d <- 0
}

func B() {
        <-c
        <-d
        e <- 0
        c <- 2
}

func C() {
        <-e
        <-c
}
\end{lstlisting}


==> lstlistings/simple_global_protocol_guarded_implementation_lstlisting_overlay2.tex <==
\begin{lstlisting}[style=base,caption={An implementation that satisfies the global protocol \eqref{eq:global protocol race-free}.},label={lst:simple global protocol guarded implementation},multicols=2]
package main

var c = make(chan int, 2)
var d = make(chan int, 0)
var e = make(chan int, 0)

func main() {
	go A()
	go B()
	go C()
}

func A() {
	c <- 1
	@d <- 0@
}

func B() {
	<-c
	@<-d@
	@e <- 0@
	c <- 2
}

func C() {
	@<-e@
	<-c
}
\end{lstlisting}


==> lstlistings/simple_global_protocol_implementation_lstlisting.tex <==
\begin{lstlisting}[label={lst:simple global protocol implementation},multicols=2]
package main

var c = make(chan int, 2)

func main() {
        go A()
        go B()
        go C()
}

func A() {
        c <- 1
}

func B() {
        <-c
        c <- 2
}

func C() {
        <-c
}
\end{lstlisting}

